Value-based Resource Matching with Fairness Criteria: Application to Agricultural Water Trading

Optimal allocation of agricultural water in the event of droughts is an important global problem. In addressing this problem, many aspects, including the welfare of farmers, the economy, and the environment, must be considered. Under this backdrop, our work focuses on several resource-matching problems accounting for agents with multi-crop portfolios, geographic constraints, and fairness. First, we address a matching problem where the goal is to maximize a welfare function in two-sided markets where buyers' requirements and sellers' supplies are represented by value functions that assign prices (or costs) to specified volumes of water. For the setting where the value functions satisfy certain monotonicity properties, we present an efficient algorithm that maximizes a social welfare function. When there are minimum water requirement constraints, we present a randomized algorithm which ensures that the constraints are satisfied in expectation. For a single seller--multiple buyers setting with fairness constraints, we design an efficient algorithm that maximizes the minimum level of satisfaction of any buyer. We also present computational complexity results that highlight the limits on the generalizability of our results. We evaluate the algorithms developed in our work with experiments on both real-world and synthetic data sets with respect to drought severity, value functions, and seniority of agents.

==> scratch.tex <==
\para{Buyer satisfaction} For the synthetic networks, we find welfare
maximizing solutions with the constraint that every buyer~$b$ is matched to
at least~$r(b)=r$ water units. Figure~\ref{fig:fairness} shows the decrease
in welfare as~$r$ increases. A value of zero on the y-axis corresponds to
an infeasible problem instance. We note that for lower~$\delta$, the loss
in welfare is large as~$\lambda$ increases.  In light of the fairness
results, we have plotted buyer satisfaction in Figure~\ref{fig:sat} for
water unit size of 10. We observe that for both the datasets, the general
satisfaction levels are low for~$\delta<0.5$.  We see some outliers with
100\% satisfaction. Upon inspection, these buyers typically have a single
unit requirement. We note that for \touchet{10}, the average buyer
satisfaction jumps to $\approx0.5$ at~$\delta=0.6$. There are low-valued
agents with water available at~$\delta\ge0.5$ who can lead to an increase
in trade. We observe that welfare is not indicative of buyer satisfaction
as it only depends on the total value and total quantity of trade. Further,
it is challenging to guarantee a minimum number of water units to most
buyers due to the fact that, in many scenarios, there are no compatible
sellers for most buyers. Therefore, with the additional constraints of
lower bounds as in Section~\ref{sse:maxwelfarefair}, this will mostly lead
to infeasible instances. Next, we note that the mean or median buyer
satisfaction need not increase as~$\delta$ increases. As~$\delta$
increases, the number of buyers decreases. Hence, it is possible that for
the remaining  buyers, the buyer satisfaction is low.  This explains the
decrease  in buyer satisfaction for \yakima{10} from~$\delta=0.3$
to~$\delta=0.4$.

In Figure \ref{fig:beta}(left), we see that as $\beta$ increases, the Social Welfare increases linearly. This makes sense since $\beta$ multiplies both parts of the welfare function. In Figure~\ref{fig:beta}(right), we see that as the difference between the low and the high beta values increases more noise is added to the graph. 
In Figure \ref{fig:delta}, social welfare is low for high or low values of $\delta$ and high for values around the average. This is because the number of buyers and sellers around the average is similar. When there are very few sellers and many buyers, or the opposite, lower amounts of trade can occur.
Figure~\ref{fig:lambda} shows that greater values of $\lambda$ are responsible for better welfare. This occurs since higher values of lambda cause more buyers to be high-valued, increasing the positive part of the welfare function.
Finally, in Figure~\ref{fig:N}, we see that as the number of agents increases, the welfare increases. This is because more trading can be performed in greater markets.


\begin{figure}[t]
    \centering          
    \includegraphics[width=0.45\textwidth]{figs/gamma.pdf}
    \caption{\label{fig:lambda}
    Results for the synthetic graphs for $N=10$, $\beta_{low}=0.3$, $\beta_{high}=0.7$ and $\delta=0.5$.
    Y-axis is the computed social welfare and the X-axis is for $\lambda$.}       
\end{figure}

\begin{figure}[t]
    \centering          
    \includegraphics[width=0.45\textwidth]{figs/N.pdf}
    \caption{\label{fig:N}
    Results for the synthetic graphs for $\beta_{low}=0.3$, $\beta_{high}=0.7$, $\lambda=0.5$ and $\delta=0.5$.
    Y-axis is the computed social welfare and the X-axis is the number of agents.}
\end{figure}


%% We use a logistic function to model value functions for both buyers and
%% sellers. 
%% we will use~$\valfun_x(\ell) =
%% \frac{2\beta}{1+e^{\ell-1}}$ for~$\ell=1,\ldots,k$.  For sellers


\begin{figure}[t]
    \centering          
    \includegraphics[width=0.32\textwidth]{figs/heatmap_0.1.pdf}
    \includegraphics[width=0.32\textwidth]{figs/heatmap_0.5.pdf}
    \includegraphics[width=0.32\textwidth]{figs/heatmap_0.9.pdf}
    \caption{\label{fig:heatmaps}
    Results for the synthetic graphs; Y-axis is for $\beta_{high}$($\beta_{low}$ is set to 1), X-axis is $\delta$, and the heat is the Social Welfare. Different maps are for different values of Gamma. }
\end{figure}
\subsection{Results on Real Datasets}

\begin{figure}[t]
    \centering          
    \includegraphics[width=0.48\columnwidth]{figs/touchet.pdf}
    \includegraphics[width=0.48\columnwidth]{figs/yakima.pdf}
    \caption{\label{fig:real}
    Results for the Touchet (left) and Yakima (right) datasets; Y-axis is for welfare, X-axis is the capacity in percent. }
\end{figure}
\subsection{Buyer's perspective}
All the problems such as (i)~all buyers satisfied? (ii)~max. number of
buyers satisfied, and (iii)~partial satisfaction will be included
depending on the progress made in the above section.
Existing results can be included if they fit into the story. For example,
healthy streamflows are essential for providing habitat for fish and
wildlife. Agencies corresponding to ecology, forestry, fishery, etc. buy
water from farmers to retain minimum stream flow
(\url{https://apps.ecology.wa.gov/publications/documents/1711002.pdf}).
The first set of problems corresponds to maximizing the following welfare
function for a trading assignment~$\trade$:~$\welfare(\trade) = \sum_{x\in
X} \valfun_x(v_x) - \sum_{y\in Y} \valfun_y(v_y)$, where~$v_x$ and~$v_y$
are the total trade volume for the buyer and seller in~$\trade$.  We first define the
\maxwelfare{} problem.
%%
\begin{problem}[Maximum Welfare Water Trading \maxwelfare]
\label{prob:maxwelfare}
Given sets of buyers~$X$ and sellers~$Y$, associated value functions, and a
compatibility graph~$G(X,Y,E)$, find a trading assignment~$\trade^*$ that
maximizes the welfare function~$\welfare(\cdot)$ subject to the following
priority constraints: (i)~each buyer~$x$ buys a total of~$v_x$ units which
is at most its requirement~$\rho_x$ with a cost~$\kappa_x=\sum_{(x,y,p)\in
\trade}p\le\valfun_x(v_x)$ and (ii)~each seller~$y$ sells a total of~$v_y$
units which is at most its capacity~$c_y$ with a price~$p_y\ge
\valfun_y(v_y)$.
\end{problem}
%%
We consider a more restricted version of the problem in the disaggregated
volumes setting. Here, for a disaggregated volumes trading assignment~$\trade$,
the \emph{disaggregated volumes welfare function} is defined as
follows:~$\uwelfare(\match) = \sum_{(w^x_i,w^y_j)\in
\match}\uvalfun_x(i)-\uvalfun_y(j)$.
%%
\begin{remark}
We note that there is a natural relationship between the general framework
and the disaggregated volumes framework. Given a value function, a
unit-value function can be derived as a finite difference of the value
function. For a buyer~$x$,~$\uvalfun_x(1)=\valfun_x(1)$ and
for~$r\in\{2,\ldots,\rho_x\}$,
$\uvalfun_x(i)=\valfun_x(r)-\valfun_x(r-1)$. A similar relationship holds
for sellers as well.  It is also to be noted that the disaggregated volumes
framework has a stricter constraint than the general framework with regard
to price satisfaction. For example, consider the following value function
for a buyer~$x$:~$\valfun_x(1)=4$ and~$\valfun_x(2)=5$. The corresponding
unit-value function is~$\uvalfun_x(1)=4$ and~$\uvalfun_x(2)=1$.
In the general framework, the buyer's requirement of two units can be
satisfied by two sellers, one with a price of~$3$ and the other with a
price of~$2$. In the disaggregated volumes framework however, the buyer
will not pay more than~$1$ for the second water unit. In this sense, the
number of possibilities for buyer satisfaction could be fewer in this case.
\end{remark}
\subsection{Disaggregated volumes framework}
Here, we consider a restricted version of the framework where water is
traded in single units. Each seller's volume and buyer's requirement is
disaggregated into water units, each unit is treated as a separate entity 
associated with a value or price, and each unit is sold separately subject to some
constraints. Let a water unit be denoted by~$w$.  For a buyer~$x$ with
requirement~$\rho_x$, we consider an ordering of the water
units~$\Gamma_x=(w^x_1,w^x_2,\cdots,w^x_{\rho_x})$. For~$1\le i\le \rho_x$,
the \emph{unit-value function}~$\uvalfun_x(i)$ assigns a value or price to
water unit~$w^x_i$. Similarly, for a seller~$y$ with capacity~$c_y$, we
consider an ordering~$\Gamma_y=(w^y_1,w^y_2,\cdots,w^y_{c_y})$ and the
corresponding unit-value function.

A trading assignment~$\trade$ is specified by a
set of tuples~$(x,y,p)$, where~$x\in X$,~$y\in Y$, and~$v\in
\integers_{>0}$ is the volume of water owned by~$y$ that is assigned
to~$x$. \textcolor{red}{mw: I am a little confused by the part of the definition where it says $v$ is the volume of water owned by $y$ that is assigned to $x$, but $v$ does not appear in the tuple -- $p$ does, and $p$ was earlier defined as the number of water units required by $x$ (which, depending on the experiment selected, may be satisfied by multiple sellers.) Am I overlooking something here?}

\paragraph{Value function.} Each buyer is associated with a value function
that associates every unit of of water with the maximum price the buyer is
willing to pay. For a buyer~$x$, the value function~$\valfun_x(v)>0$ if and
only if~$v\le \rho_x$. Similarly, each seller is associated with a value or
price function that associates a volume of water with the minimum price the
seller is willing to accept. For a seller~$y$,~$\valfun_y(v)>0$ if and only
if~$v\le c_y$. For a buyer, the value function specifies the budget per
volume of water, while for the seller, it represents the minimum income per
volume of water.

%%%% Replaced this version.
\iffalse
%%%%%%%%%%%%%%%%%%%
%%
\begin{figure*}[htb]
    \centering
    \includegraphics[width=.8\textwidth]{figs/example_sketch.jpeg}
    \caption{Example}
    \label{fig:example}
\end{figure*}
%%
%%%%%%%%%%%%%%%%%%%
\fi 


\paragraph{Value/price function.} Each buyer is associated with a value or
price function that associates a volume of water with the maximum price the
buyer is willing to pay. For a buyer~$x$, the value
function~$\valfun_x(v)>0$ if and only if~$v\le \rho_x$. Similarly, each seller
is associated with a value or price function that associates a volume of
water with the minimum price the seller is willing to accept. For a
seller~$y$,~$\valfun_y(v)>0$ if and only if~$v\le c_y$. For a buyer, the
value function specifies the budget per volume of water, while for the
seller, it represents the minimum income per volume of water.

For~$1\le i\le \rho_x$, the \emph{unit-value
function}~$\uvalfun_x(i)$ assigns a value or price to water unit~$w^x_i$.

 In this setup, we will assume that
all capacities, requirements, and trade volumes are represented in terms of
a standard unit of water, which is indivisible. This implies that~$\rho_x$
and~$c_j$ are positive integers.
\begin{figure}[t]
    \centering          
    \includegraphics[width=.23\textwidth]{figs/beta.pdf}
    \includegraphics[width=.23\textwidth]{figs/betadiff.pdf}
    \caption{\label{fig:beta}
    Results for the synthetic graphs for $N=10$, $\delta=0.5$ and $\lambda=0.5$.
    Y-axis is the computed social welfare and the X-axis(left) is for $\beta$; in this graph all $\beta$ values are identical. X-axis(right) holds both high and low values of $\beta$.
    }
\end{figure}

\begin{figure}[t]
    \centering          
    \includegraphics[width=0.45\textwidth]{figs/delta.pdf}
    \caption{\label{fig:delta}
    Results for the synthetic graphs for $N=10$, $\beta_{low}=0.3$, $\beta_{high}=0.7$ and $\lambda\in{0.1,0.5,0.9}$.
    Y-axis is the computed social welfare and the X-axis is for $\delta$.}   
\end{figure}

